NoviCode: Generating Programs from Natural Language Utterances by Novices

Current Text-to-Code models demonstrate impressive capabilities in generating executable code from natural language snippets. However, current studies focus on technical instructions and programmer-oriented language, and it is an open question whether these models can effectively translate natural language descriptions given by non-technical users and express complex goals, to an executable program that contains an intricate flow - composed of API access and control structures as loops, conditions, and sequences. To unlock the challenge of generating a complete program from a plain non-technical description we present NoviCode, a novel NL Programming task, which takes as input an API and a natural language description by a novice non-programmer and provides an executable program as output. To assess the efficacy of models on this task, we provide a novel benchmark accompanied by test suites wherein the generated program code is assessed not according to their form, but according to their functional execution. Our experiments show that, first, NoviCode is indeed a challenging task in the code synthesis domain, and that generating complex code from non-technical instructions goes beyond the current Text-to-Code paradigm. Second, we show that a novel approach wherein we align the NL utterances with the compositional hierarchical structure of the code, greatly enhances the performance of LLMs on this task, compared with the end-to-end Text-to-Code counterparts.

==> pages/archive/2_the_challenge_old.tex <==
\section{The Challenge: Technical Code for Non-Technical Users}
In the landscape of current Text-to-Code tasks, genuine natural language programming remains a distant dream. 
Models for translating text to code are primarily designed with a programmer-centric perspective in mind, rather than being optimized for catering to the needs of novice users.
Evaluation methods for code synthesis models present additional challenges that are magnified in the case of evaluating synthesized programs from plain language instructions of non-programmers.

%We address the challenge of enabling novices and non-programmers to generate intricate programs using plain-language descriptions, highlighting the limitations of current models reliant on technical jargon-heavy datasets. Evaluating NLP-based code generation models presents additional challenges.

%These models consistently fall short when tasked with non-technical NL translations to elucidate intricate code execution.
%\reut{do you actually have evidence for that? which and where?} \asaf{we do - in the experiment section, but I agree with you that line was too conclusive and generic} \asaf{Please see revision.}
%Recent advancements still remain confined to aiding adept programmers,
%Recent advancements still remain confined to the current Text-to-Code paradigms, primarily catering to technical jargon and programmer-specific discourse, while often overlooking the intuitive and natural language nuances of novice or non-programmer users.
%\reut{"confined to aiding adept programmers" is too vague, abstract, and generally not precise enough} \asaf{Please see revision.} %rather than democratizing code generation for the wider audience, including novices and those unfamiliar with programming paradigms.

Considering these challenges, we present a new task to synthesize intricate code from a non-technical user description of a complex program.

\subsection{How to program in natural language?}
We aim to empower novices and non-programmers to craft complex programs using plain-language descriptions. In our pursuit of this goal, we consider two pivotal factors: the skill level of users in framing their NL requests and the complexity of the described programs. 
\asaf{add a paragraph on the difference of using NL to describe code between programmer and novices. This para should detail the required skillset (or missing skills) and the difference between the two types of novices/programmers}
The skill level reflects the user's familiarity with technical jargon, while complexity pertains to the involved control flow structures within the elicited program code. These two factors are important in the availability of a dataset for the task of generating complex code programs from plain language descriptions by novices.

The example ''\textit{Wake me up 15 minutes earlier if it snows in the morning}`` utilizes straightforward, everyday language, making it accessible and easy to articulate without specialized skill. Nonetheless, it elicits a complex \asaf{detail above/before (standalone) complex vs simple} program as it implies a conditional flow in execution.
To highlight the stark contrast in examples found in typical text-to-code datasets, consider: "\textit{Start a server on port 8080}" \asaf{simple} or "\textit{Find the largest prime factor of number n}" \asaf{find a different example that better requires programming skill}. These instances leverage technical directives and suggest complex programs, involving underlying flow structures, all while concealing the intricacies beneath specialized terms and concepts familiar primarily to experienced programmers.

Most existing datasets tailored for code synthesis originate from GitHub repositories' code comments or StackOverflow Q\&A pairs. Thus, predominantly showcasing specific programming skill level while varying in their exhibited program complexity. The CoNaLa Dataset \citep{DBLP:journals/corr/abs-1805-08949} contains programming questions from Stack Overflow along with code solutions. The CONCODE dataset \citep{DBLP:journals/corr/abs-1808-09588}, the CodeSearchNet Corpus \citep{DBLP:journals/corr/abs-1909-09436}, and the CodeXGLUE dataset \citep{lu2021codexglue} were constructed using code-comment pairs from GitHub across numerous domains in various programming languages.
This introduces an inherent challenge\asaf{not challenge -> properties}: these datasets often contain descriptions created by experienced programmers, rich in specialized jargon and nuanced programming concepts like algorithms (e.g. \textit{bubble sort}), methodologies (e.g. \textit{authentication}), and network concepts \textit{client-server}. Moreover, these descriptions typically reference specific terminologies stated in terms of the underlying software ontology, including terms like \textit{dictionary}, \textit{port}, and \textit{file system}.

Consequently, the NL requests in these datasets are articulated in a technically advanced language used by skilled programmers. The complexity of the code translated from these requests mirrors \asaf{not true -- complex and non-complex} the depth of concepts, ideas, and terms expressed within them.

Datasets of plain-language descriptions from novice users are commonly found in Task-oriented Dialog Systems, which are used by virtual assistants. Notable Task-oriented datasets are TOP \citep{DBLP:journals/corr/abs-1810-07942} and TOPv2 \citep{DBLP:journals/corr/abs-2010-03546} datasets. However, NL utterances in these datasets typically translate to simpler program codes, lacking the complexity we are targeting.

Therefore, we recognize an unaddressed gap in the landscape of code synthesis and generation that current models fail to handle (figure \ref{fig:magic-quadrant}).

%The first challenge in achieving actual NL programming lies in the data that current code synthesis models rely on. We aim to empower novices and non-programmers to craft intricate code from plain-language descriptions. However, the predominant datasets for this purpose are derived from GitHub repositories' code comments and code pairs, or StackOverflow Qֿֿֿֿֿֿֿֿ\&A. This creates an intrinsic problem: the descriptions generated by adept programmers, laden with specialized jargon based on nuanced software programming concepts. 

%Furthermore, code comments and functions docstrings in massive code-based data (e.g. GitHub public data) appear in a domain-specific dialect, which is highly structured with repetitive templates \citep{10.1145/3324884.3416546}. Moreover, developers often struggle with creating meaningful comments, which are frequently neglected (\citealp{de2005study}, \citealp{fluri2007code}). Consequently, the limited expressivity and questionable quality may restrict the models' adaptability to the language novices use for complex programming  (figure \ref{fig:magic-quadrant}). 

\begin{figure}
    \centering
    \begin{center}
    \begin{tikzpicture}
    \begin{axis}[
        axis lines=center,
        xtick=\empty,
        ytick=\empty,
        xmin=-10,
        xmax=10,
        ymin=-10,
        ymax=10,
        xlabel=\textbf{Skill level},
        ylabel=\textbf{Code complexity},
        x label style={at={(axis description cs:0.88,0.5)},anchor=north},
        y label style={at={(axis description cs:0.5,1.0)},anchor=west}
    ]
    
    \begin{pgfonlayer}{background}
        \fill[pastelyello!20] (axis cs:-10,0) rectangle (axis cs:0,10);  % Top left quadrant
        \fill[deepgray!20] (axis cs:0,0) rectangle (axis cs:10,10);    % Top right quadrant
        \fill[lightgray!20] (axis cs:-10,0) rectangle (axis cs:0,-10);   % Bottom left quadrant
        \fill[deepgray!20] (axis cs:0,0) rectangle (axis cs:10,-10); % Bottom right quadrant
    \end{pgfonlayer}
    
    \node at (axis cs:5,5) {1};
    \node at (axis cs:-5,5) {2};
    \node at (axis cs:-5,-5) {3};
    \node at (axis cs:5,-5) {4};
    
    \node[anchor=east,font=\small] at (axis cs:-5.5,1) {Novices};
    \node[anchor=west,font=\small] at (axis cs:3.25,1) {Programmers};
    \node[anchor=south,font=\small] at (axis cs:0,-9) {Simple};
    \node[anchor=north,font=\small] at (axis cs:0,9) {Complex};
    
    \end{axis}
    \end{tikzpicture}
    \end{center}
    \caption{Identifying a void in the landscape of code synthesis models. Our task focuses on NL requests of novice users describing complex programs (quadrant 2).}
    \label{fig:magic-quadrant}
\end{figure}

%In addition, the terminology used in these datasets is correlated with problems in software programming domains. Specialized jargon and nuanced software programming concepts in NL sentences are stated in terms of the underlying ontology. Concepts, terms, and words (e.g. \textit{bubble sort}, \textit{authentication}, \textit{server}, etc.), and in conjunction with the utilization of contextualized data-structures ontology (e.g. \textit{dictionary}, \textit{port}, \textit{file system}, etc.) bias the success of a code synthesis task towards this realm (of software programming paradigms).

\subsection{How to evaluate code generated from natural language?}

%Evaluating code generation tasks in NLP is challenging due to the nuanced nature of code semantics, the need for functional correctness, and the diversity of valid code solutions for a single prompt. \reut{rephrase}

Code generation models have traditionally been assessed by comparing them to a reference code using metrics such as BLEU scores \cite{papineni-etal-2002-bleu}. However, BLEU is only considering the token match and ignoring the
importance of keywords, syntactic accuracy, and semantic correctness of the generated program. 
CodeBLEU \cite{DBLP:journals/corr/abs-2009-10297} enhances BLEU by incorporating crucial code-related features such as syntactic and semantic similarity, dataflow, and variable misuse. Though, despite its improvements, CodeBLEU still relies on string-match based metrics and thus fall short in accounting for the vast space of programs that are functionally equivalent to a reference solution. \asaf{shorten}

As a result, recent works in code synthesizing turned to evaluating models through the functional correctness of the generated code. In this line of work, a dataset sample is considered correct if it passes a set of unit tests. 
HumanEval \citet{DBLP:journals/corr/abs-2107-03374} is a notable work in this direction. HumanEval measures functional correctness for programs synthesized from docstrings. It presents a dataset of hand-written unit tests for programming problems. The programming problems in HumanEval are like those in programmers' datasets such as Github. 
However, we seek to evaluate problems articulated in plain English and describe complex programs. Generating a dataset of plain language descriptions of complex programs and their respective unit tests suites is harder as there are no datasets in place, which we can source problems from. Also, generating such dataset requires the participation and orchestration of multiple parties -- both non-programmers for supplying the descriptions, and programmers for writing the unit tests.





%We aim to enable novices and non-programmers to craft complex programs through natural language descriptions. In our pursuit we consider two pivotal factors: the language used in these descriptions and the complexity of the described programs.
%Programmers and novices formulate code descriptions distinctly due to their varied levels of expertise and familiarity with technical jargon. Code synthesis models are trained, tuned, and evaluated using program descriptions articulated through utterances crafted by programmers.
%Novices provide intuitive, everyday language descriptions. Programmers' descriptions, on the other hand, are often rich in specialized jargon and nuanced programming concepts like algorithms (e.g. \textit{binary search}), methodologies (e.g. \textit{authentication}), and concepts (e.g. \textit{client-server}). Moreover, these descriptions typically reference specific terminologies stated in terms of the underlying software ontology, including terms like \textit{DataFrame}, \textit{port}, and \textit{file system}.
%In order to effectively program using natural language, an utterance encapsulating a desired functionality of a program should be expressible without demanding an advanced programming skill level. Furthermore, the description should not limit the projected intricacies of the logical flow within the resultant program.
%The primary challenge we identify is the language utilized in program descriptions. The skill level of individuals crafting the utterances inherently shapes the language. Most existing datasets tailored for code synthesis originate from GitHub repositories’ code comments or StackOverflow Q\&A pairs. 
%Non-programmers use everyday, plain language to provide descriptions for programs. Datasets of plain-language descriptions from novice users are commonly found in Task-oriented Dialog Systems, which are used by virtual assistants. However, NL utterances in these datasets typically translate to simpler program codes, lacking the complexity we are targeting.

==> pages/archive/8_method_old.tex <==
\section{Modeling Text-to-Code Structured Alignment} \label{section:method}

\yg{this section is not clear to me. (a) it is not about modeling. it is also not about alignment. it is about transforming the problem somehow. (b) how does this work? you generate the cAST, and then what? how does the cAST turn into code? this part is very much missing. (c) how does the cAST look like?}

Code synthesis models aim to convert natural language descriptions directly into executable code, often using sequence-to-sequence architectures where the source language is a human language and the target language is a programming language.

We hypothesize that explicitly representing the structure of the target complex program, through a hierarchical tree expressing the compositional control flow structures expressed in the code, can enhance the code generation process of complex programs from NL. This method has the potential to improve compositional generalization relative to standard end-to-end text-to-code methods \citep{DBLP:journals/corr/abs-2009-06040}.

We present a novel approach for complex code generation from novice NL instructions, which relies on aligning utterances to the syntactic structures of the denoted code. 
%We aim to identify patterns within the program code corresponding to specific segments of the NL description, aligning the two effectively. 
To this end, we establish a representation format for the corresponding program code.%, as we detail below.
Our method creates a hierarchical representation of the program code based on its Abstract Syntax Tree (AST). 
ASTs provide a structured, hierarchical representation of the code, which should be easier for models to learn and generate. 
Control flow logic is reflected in the branches and nodes of the AST, thus allowing the model to focus more on the logic and flow of the complex program rather than syntax (e.g. proper keywords, symbols, and indentation), reducing the complexity of the output space. 

On top of that, we define a compact  AST (denoted cAST) by only retaining the control flow logic structures, such as sequences, conditions, and loops, in a tree form. 
To create the dense tree structures, we revert basic operations such as variable assignments or function calls to their fundamental code syntax. These elements are transformed from their AST hierarchical representation to appear as leaves in the tree's code form.
%(Section \ref{subsection:method.code}) \reut{why not move here the representation}

%% discuss the eval set in conjunction with a trained model. Should be discussed in the experiment part!

%\paragraph{Formal Settings}
%Formally, given a natural language utterance $x$, our goal is to convert $x$ into a surface code $y$. 
%We approach this problem by mapping the NL utterance $x$ to the code-related logical form, $z$, that can be deterministically translated into the surface code $y$. 
%To support our pipeline we define a downstream probabilistic model for generating the intermediate form $\hat{z}$ given $x$: $\hat{z} = \text{argmax}_z P(z|x)$. %\reut{dont you need an argmax somehere here?} 
%$\hat{z}$ is then converted into a surface code $\hat{y}$. 
%We wish to compute $p(z|x)$, which we approximate using a sequence-to-sequence network from the NL utterance sequence $x$ into a linearized tree form of $\hat{z}$.\yg{if we are not actually solving the argmax or even anything remotely close to it, what is the purpose/benefit of writing it in this form?}

%\subsection{Program Code Intermediate Representation} \label{subsection:method.code}

%Given a syntactically correct code, Abstract Syntax Trees (ASTs) manifest a tree structure 
%%that reflects the hierarchical \yg{is reflecting complexity a good thing? why?} of the corresponding program and the order in which it is executed. ASTs 
%provide a systematic representation of the structure of a program code, highlighting relationships between its elements. 
%Control flow logic, which directs the order of operations within a program, is reflected in the branches and nodes of the AST.%, enabling a clear visualization of the execution path the program follows. %\reut{need to explicitly equate the AST with the z object}

Formally, given a natural language utterance $x$, our goal is to convert $x$ into a surface code $y$. 
We approach this problem by mapping the NL utterance $x$ to the code-related logical form, $z$, that can be deterministically translated into the surface code $y$. 
Our model learns the transformation $x \rightarrow z$. 
We do so using sequence-to-sequence models with a greedy decoder outputting a linearized bracket notation representing the hierarchical structure, termed $z$. 
Last, this intermediate representation $z$ can be deterministically converted\footnote{We offer a tool that transforms compacted ASTs into their standard forms. These ASTs are then translated into actual code using the official packages available for each programming language.} back into a surface code $y$.

We note that previous works (\citealp{yin-neubig-2017-syntactic}, \citealp{yin2018tranx}) also utilized ASTs to synthesize code better. Yet, these works model code generation as a series of classification problems of grammar rules required to reconstruct the AST. Our method uses the hierarchical tree form directly as a vehicle to correctly generate hierarchical code structures.


%This format allows for a clearer correlation between the code-condensed ASTs and their matching NL utterance spans. It simplifies the process of matching spans in the NL description with their equivalent code segments. For instance, a conditional clause in the NL description can be directly aligned with an \texttt{If} segment in the code's AST.
%The rules and labels are further discussed in Appendix \ref{appendix:code-rep}.\reut{no appendix allowed in TACL submissions - remove this line, and remove the appendix}
%\yg{i don't understand what the method actually does: how is the code represented as AST? the figure doesn't help, it should a tree, but how do we feed a tree to a sequence model / LM?}

% \newcommand{\smallcircled}[1]{
%   \tikz[baseline=(char.base)]{
%     \node[shape=circle, draw, inner sep=0.5pt, font=\footnotesize] (char) {#1};
%   }
% }
% \begin{figure}[t]
%     \centering
%     \textit{If it rains tomorrow then text Alice}
%     \newline
%     \begin{tikzpicture}
%         \draw[dashed, line width=0.25pt, black] (-4,0) -- (4,0);
%     \end{tikzpicture}
%     \footnotesize
%     \textbf{Dense AST}
%     \\
%     \vspace{0.2cm}
%     \begin{tikzpicture}[
%         level distance=0.75cm, font=\footnotesize,
%         level 1/.style={sibling distance=2.0cm},
%         level 2/.style={sibling distance=1.85cm},
%         level 3/.style={sibling distance=1.254cm},
%         level 4/.style={sibling distance=4cm},
%         level 5/.style={sibling distance=5cm},
%         level 6/.style={sibling distance=1.25cm},
%         level 7/.style={sibling distance=1.25cm},
%         level 8/.style={sibling distance=1.25cm},
%         level 9/.style={sibling distance=1.25cm},
%         triangle/.style={isosceles triangle,draw,shape border rotate=90,    minimum height=10mm, minimum width=15mm,yshift=-1.5cm
%         },
%     ]
%         \node {Module}
%         [child anchor=north]
%         child { node[triangle] (tri1) {} }
%         child { node {If} 
%             child { node {test} 
%                 child { node { $x$ } }
%             }
%             child { node {body}
%                 child { node[triangle] (tri2) {} }
%             }
%         }
%         ;
%         % \node at (tri1.center) {\smallcircled{1}};
%         % \node at (tri2.center) {\smallcircled{2}};
%         % \node at (0.5, 1) {\textbf{Dense AST}};
%         \node at (tri1.south) [yshift=-0.3cm] { Lines 1-6 };
%         \node at (tri2.south) [yshift=-0.3cm] { Lines 9-14 };
%     \end{tikzpicture}
    
%     \begin{tikzpicture}
%         \draw[dashed, line width=0.25pt, black] (-4,0) -- (4,0);
%     \end{tikzpicture}

%     \centering
%     \small % Set the font size
%     \textbf{Code}
%     \vspace{0.2cm}
%     \begin{lstlisting}[style=python]
% weather_cond = WeatherCondition.resolve_from_text('rains')
% date_time = DateTime.resolve_from_text('tomorrow')
% weather_forecast = WeatherForecast.find_weather(
%     weather_cond=weather_cond, 
%     date_time=date_time
% )
% x = bool(weather_forecast)
% if (x):
%     message_content_type = MessageContentType.resolve_from_text('text')
%     recipient = Contact.resolve_from_text('Alice')
%     Message.send_message(
%         recipient=recipient, 
%         message_content_type=message_content_type
%     )
% )
%     \end{lstlisting}
% \caption{This figure illustrates our proposed alignment method from a language description span to an AST hierarchical tree form. Top: the utterance \textit{"If it rains tomorrow then text Alice"}. Middle: Our proposed condensed version of an AST as an intermediate structural form of the target code. Bottom: The resultant or expected code. }
%     \label{figure:lang-rep}
% \end{figure}

